Poisoning Web-Scale Training Datasets is Practical

Deep learning models are often trained on distributed, web-scale datasets crawled from the internet. In this paper, we introduce two new dataset poisoning attacks that intentionally introduce malicious examples to a model's performance. Our attacks are immediately practical and could, today, poison 10 popular datasets. Our first attack, split-view poisoning, exploits the mutable nature of internet content to ensure a dataset annotator's initial view of the dataset differs from the view downloaded by subsequent clients. By exploiting specific invalid trust assumptions, we show how we could have poisoned 0.01% of the LAION-400M or COYO-700M datasets for just $60 USD. Our second attack, frontrunning poisoning, targets web-scale datasets that periodically snapshot crowd-sourced content -- such as Wikipedia -- where an attacker only needs a time-limited window to inject malicious examples. In light of both attacks, we notify the maintainers of each affected dataset and recommended several low-overhead defenses.

==> tables/downloads.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{@{}l|c c c c c}
    \toprule
        \makecell{\textbf{Dataset}\\\textbf{Name}} & \makecell{\textbf{Downloads}\\\textbf{Per Week}} & \makecell{\textbf{\% Unique}} & \makecell{\textbf{\% Sequentially} \\ \textbf{Downloaded}} & \makecell{\textbf{Download}\\\textbf{Time (hours)}} & \makecell{\textbf{Unique}\\\textbf{Requests}}\\
        \midrule
        LAION-5B~\cite{schuhmann2022laion} & TODO &\\
        COYO-700M~\cite{kakaobrain2022coyo-700m} & TODO & \\
        LAION-400M~\cite{schuhmann2021laion} & TODO &\\
        WiT~\cite{srinivasan2021wit} & TODO \\
        CC-12M~\cite{changpinyo2021conceptual} & TODO \\
        CC-3M~\cite{sharma2018conceptual} & TODO \\
        VGG Face~\cite{parkhi2015deep} & TODO \\
        Facescrub~\cite{ng2014data} & TODO & \\
        Pubfig~\cite{kumar2009attribute} & TODO & \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Many models would have been poisoned via our attacks}, because they are downloaded online for model training. Results obtained via passive monitoring of the three most popular expired domains for each dataset. Observe that all datasets are often downloaded in a predictable sequential pattern and slow enough for frontrunning to be effective. Measurements taken between  \cc{todo}}
    \label{tab:download-impact}
\end{table*}

==> tables/editrates.tex <==
\stepcounter{numheaders}
\stepcounter{numheaders}
\begin{table*}[]
    \centering
    % @{\hspace{\tabcolsep}}
    {\setlength{\tabcolsep}{5pt}
    \begin{tabular}{@{}L|S[table-format=3.2]@{}cccccccc}
    \toprule
        \textbf{Dataset} & \textbf{Size} & \textbf{Release} & \textbf{Cryptographic} 
        & \textbf{Data} & \textbf{Data} & \textbf{Data} & \textbf{Data} & \textbf{Downloads} \\%
        \textbf{Name} & \textbf{($\times 10^6$)} & \textbf{Date} & \textbf{Hash?} 
        & \textbf{Editable*} & \textbf{Expired} & \textbf{Buyable} & \textbf{Poisonable} &  \textbf{Per Week} \\
        \midrule
        
        LAION-2B-en~\cite{schuhmann2022laion} & 2323 & 2022 & \xmark\makebox[0.5em][r]{\footnote{LAION-5B released a ``joined'' version of this dataset with a cryptographic hash over the URL (not the \emph{contents} of the URL) and Caption, and as such does not protect the integrity of the actual image.\label{5bnote}}} & 
        0.40\% & 0.29\% & $\ge$ 0.02\% & TODO & TODO\\
        
        LAION-2B-multi~\cite{schuhmann2022laion} & 2266 & 2022 & \xmark\makebox[0.5em][r]{\footnotemark[\getrefnumber{5bnote}]} & 
        0.37\% & 0.55\% & $\ge$ 0.03\% & TODO & TODO\\
        
        LAION-1B-nolang~\cite{schuhmann2022laion} & 1272 & 2022 & \xmark\makebox[0.5em][r]{\footnotemark[\getrefnumber{5bnote}]} & 
        0.58\% & 0.37\% & $\ge$ 0.03\% & TODO & TODO\\
        
        COYO-700M~\cite{kakaobrain2022coyo-700m} & 747 & 2022 & \xmark\makebox[0.5em][r]{\footnote{COYO-700M images are distributed with a PHash which does validate benign image changes, but is not adversarially robust \cite{jain2022adversarial}}} & 
        0.13\% & 1.51\% & $\ge$ 0.15\% & TODO & TODO \\
        
        LAION-400M~\cite{schuhmann2021laion} & 408 & 2021 & \xmark\makebox[0.5em][r]{} & 
        0.56\% & 0.71\% & $\ge$ 0.06\% & 0.62\% & TODO\\

        CC-12M~\cite{changpinyo2021conceptual} & 12 & 2021 & \xmark\makebox[0.5em][r]{} & 
        0.11\% & 1.19\% & $\ge $ 0.15\% & 0.26\%\\
        
        CC-3M~\cite{sharma2018conceptual} & 3 & 2018 & \xmark\makebox[0.5em][r]{} & 
        0.06\% & 1.04\% & $\ge$ 0.11\% & 0.17\%\\
        
        VGG Face~\cite{parkhi2015deep} & 2.6 & 2015 & \xmark\makebox[0.5em][r]{} & 
        1.78\% & 3.70\% & $\ge$ 0.23\% & 2.01\%\\
        
        Facescrub~\cite{ng2014data} & 0.10 & 2014 & \xmark\makebox[0.5em][r]{} &
        2.34\% & 4.51\% & $\ge$ 0.79\% & 3.13\%\\
        
        Pubfig~\cite{kumar2009attribute} & 0.06 & 2010 & \cmark\makebox[0.5em][r]{\footnote{Pubfig was not intiaially released with hashes, but two months after the initial release in Version 1.2 of the dataset, the authors added MD5 hashes TODO.}} & 
        0.29\% & 6.48\% & $\ge$ 0.48\% & 0.77\%\\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Most recently-published large datasets are vulnerable to \emph{retroactive poisoning} attacks.} \at{next sentence reads weird. Consider, "prior to us notifying them of this vulnerability"} Datasets that were vulnerable to retroactive poisoning prior to us have been notified of this vulnerability. Observe that all have $>0.01\%$ of data purchaseable, exceeding what was needed in prior work~\cite{carlini2021poisoning}. Also observe these datasets are frequently re-parsed, i.e., users of the data do not maintain a local version.}
    \label{tab:pointer_datasets}
    }
\end{table*}

==> tables/pubfig.tex <==

\begin{table*}[t]
\centering
\begin{tabular}{@{}lrrrr@{}}
&& &Download  & Invalid \\
Dataset & \# Images & Success & failure  & image    \\
\toprule
\texttt{pubfig} & 58795 & 35.2\% & 54.7\% & 10.2\% \\\texttt{facescrub} & 106863 & 48.5\% & 44.5\% & 7.0\% \\\bottomrule

\end{tabular}
\caption{Link rot in old image datasets, downloaded using \texttt{img2dataset} \cite{beaumont-2021-img2dataset}.
In older datasets, the proportion of images that are no longer available online is high.}
\label{tab:stats-img2dataset}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{@{}lrrrrrr@{}}
& & & Accuracy on    & Accuracy on       & Accuracy on       & Accuracy on \\
Dataset & Downloaded & Modified & modified, no crop & modified, crop  & original, no crop & original, crop \\           
\toprule
\texttt{pubfig} & 20668 & 52.4\% & 59.7\% & 55.2\% & 96.0\% & 98.2\% \\\texttt{facescrub} & 51847 & 29.4\% & 93.3\%  & 91.6\% & 97.7\% & 99.1\% \\\bottomrule

\end{tabular}
\caption{Quantifying changes on successfully downloaded images.
Modified images are those that have a different hash than the original image.
We measure the accuracy as the proportion of modified images that have a CLIP embedding close to \emph{any} of the possible labels, approximating the question "Is there a recognizable face in the image?".
The difference between cropped and uncropped images is largely due to the resized images making the crop not capture the face of the person, as in \Cref{fig:renee_zellweger}.}
\label{tab:stats-clip-hashes}
\end{table*}
